Sound Structure-Preserving Transformation for Weakly-Left-Linear Deterministic Conditional Term Rewriting Systems

In this paper, we show that the SR transformation, a computationally equivalent transformation proposed by Serbanuta and Rosu, is a sound structure-preserving transformation for weakly-left-linear deterministic conditional term rewriting systems. More precisely, we show that every weakly-left-linear deterministic conditional term rewriting system can be converted to an equivalent weakly-left-linear and ultra-weakly-left-linear deterministic conditional term rewriting system and prove that the SR transformation is sound for weakly-left-linear and ultra-weakly-left-linear deterministic conditional term rewriting systems. Here, soundness for a conditional term rewriting system means that reduction of the transformed unconditional term rewriting system creates no undesired reduction sequence for the conditional system.

==> eptcsdata.tex <==
\providecommand{\firstpage}{62}
\providecommand{\publicationstatus}{H. Cirstea, S. Escobar (Eds.): Third International Workshop on Rewriting\\ 
Techniques for Program Transformations and Evaluation (WPTE'16).
\\
EPTCS 235, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.235.5}{10.4204/EPTCS.235.5}}
\pdfoutput=1

